On the Number of Facets of Three-Dimensional Dirichlet Stereohedra III: Full Cubic Groups

We are interested in the maximum possible number of facets that Dirichlet stereohedra for three-dimensional crystallographic groups can have. The problem for non-cubic groups was studied in previous papers by D. Bochis and the second author (Discrete Comput. Geom. 25:3 (2001), 419-444, and Beitr. Algebra Geom., 47:1 (2006), 89-120). This paper deals with ''full'' cubic groups, while ''quarter'' cubic groups are left for a subsequent paper. Here, ''full'' and ''quarter'' refers to the recent classification of three-dimensional crystallographic groups by Conway, Delgado-Friedrichs, Huson and Thurston (math.MG/9911185, Beitr. Algebra Geom. 42.2 (2001), 475-507). Our main result in this paper is that Dirichlet stereohedra for any of the 27 full groups cannot have more than 25 facets. We also find stereohedra with 17 facets for one of these groups.

==> Untitled.tex <==



every crystallographic orbit $Gp$ has that property either for $G$ or for a proper subgroup of $G$, 

We take here the following convention.

 
 
 Even more so, there are four 1-parameter families of crystallographic orbits that are not orbits with trivial stabilizer for any group. They all belong to cubic groups and have stabilizers of order two with respect to the minimal groups of which they are orbits. As said above, their Dirichlet stereohedra where completely classified in~\cite{Koch73}.
See more details in the appendix, where we also show how the bounds in the previous papers of this series still hold in these cases.



 
 In the appendix we show that the bounds given in this and the previous papers still apply for stereohedra that are not fundamental domains.
  



With this convention, there are only four 1-parameter families of Dirichlet stereohedra that are not fundamental domains of the cor, for the cubic groups 

we do not know of any Dirichlet stereohedron with non-trivial stabilizer. Theorem~\ref{thm:stabilizer-subgroup} says that, if they exist, their stabilizers have order two and the group $G$ must be tetragonal or cubic. In the appendix we bound the number of facets of the Dirichlet stereohedra in these cases, showing that the results of~\cite{Bochis-Santos-2001, Bochis-Santos-2006} are still valid for them
(Theorems~\ref{thm:stabilizer-reflection} and~\ref{thm:stabilizer-tetragonal}). Among full cubic groups, Dirichlet stereohedra with non-trivial stabilizer can only (perhaps) occur in one of them, $F4_132$, and they have at most twelve facets (Theorem~\ref{thm:stabilizer-full}).


In the previous papers in this series we have assumed that \emph{our orbits have trivial stabilizer under the group $G$.} That is, if $p$ and $G$ are the point and crystallographic group that define our Dirichlet stereohedron, we assume that the only element $g\in G$ with $gp=p$ is the identity. In~\cite{Bochis-Santos-2001} that property is part of our definition of Dirichlet stereohedron. In~\cite{Bochis-Santos-2006} we do not include the property in the definition but we say (cf.~\cite[p.~92]{Bochis-Santos-2006}): \emph{We assume that $p$ has trivial stabilizer under the action of $G$, since otherwise  $Gp$ is also an orbit of a proper subgroup of $G$}. 

We have to admit that this sentence is \emph{false}, as the following example shows.

\begin{example}
\label{exm:stabilizer}
Let $G$ be the full cubic group $F23$ and let $p$ be a base point lying in the edge $13$ of the base tetrahedron (the Delone tetrahedron of the  $I$ lattice, as in the previous sections). Assume that $p$ is otherwise generic. Then, the stabilizer of $p$ has order two, generated by the rotation of order two around the edge $13$ but $Gp$ is not an orbit of any proper subgroup of $G$.

\rm
Suppose that $H\le G$ is an index two subgroup of $G$ for which $p$ has trivial stabilizer.
Since the point group of $F23$ (the direct symmetries of a regular tetrahedron) does not have any proper subgroup of index two, $H$ has the same point group as $G$, hence it is a cubic group. It is a full group, since any quarter subgroup of a full group must have index at least four (``quarter groups contain only a quarter of the rotations of order three''). That is, $H$ is a full cubic group with the same point group as $F23$ but a translational subgroup of index two. The only candidate is $I23$, but $Gp$ is not an orbit of it (see Table 2).
\end{example}



In this appendix we show that:

\begin{itemize}
\item There are few cases in which an orbit with non-trivial stabilizer for a  three-dimensional crystallographic group $G$ is not an orbit for a proper subgroup of $G$. For this to happen, $G$ must be either cubic or tetragonal and the stabilizer of the orbit must have only one non-trivial element: a rotation of order two.

\item Even in these special orbits the bounds stated in this series of paper hold for the Dirichlet stereohedra produced.

\end{itemize}

Observe, however, that in the example above the orbit $Gp$ is an orbit with trivial stabilizer for another crystallographic group $H$, except $H$ is not a subgroup of $G$. Namely, let $H$ be the product of the translational group of the lattice $F$, the inversion on any lattice point, and the rotation of order three on one of the diagonal axes of the lattice. 
In Theorem~\ref{thm:stabilizer-full} below we show that among full cubic groups this is almost always the case: 

\begin{proposition}
Except (perhaps) for a very specific 1-parametric family of orbits in the group $F4_132$, 
all orbits with non-trivial stabilizer in  
a full-cubic group $G$ are orbits with trivial stabilizer in another crystallographic group.
\end{proposition}





